Evaluation of Finetuned LLMs in AMR Parsing

AMR (Abstract Meaning Representation) is a semantic formalism that encodes sentence meaning as rooted, directed, acyclic graphs, where nodes represent concepts and edges denote semantic relations. Finetuning decoder only Large Language Models (LLMs) represent a promising novel straightfoward direction for AMR parsing. This paper presents a comprehensive evaluation of finetuning four distinct LLM architectures, Phi 3.5, Gemma 2, LLaMA 3.2, and DeepSeek R1 LLaMA Distilled using the LDC2020T02 Gold AMR3.0 test set. Our results have shown that straightfoward finetuning of decoder only LLMs can achieve comparable performance to complex State of the Art (SOTA) AMR parsers. Notably, LLaMA 3.2 demonstrates competitive performance against SOTA AMR parsers given a straightforward finetuning approach. We achieved SMATCH F1: 0.804 on the full LDC2020T02 test split, on par with APT + Silver (IBM) at 0.804 and approaching Graphene Smatch (MBSE) at 0.854. Across our analysis, we also observed a consistent pattern where LLaMA 3.2 leads in semantic performance while Phi 3.5 excels in structural validity.

==> pgfplots_styles.tex <==
    \pgfplotsset{
        width=0.8\textwidth,
        height=0.5\textwidth,
        grid=none,
        every axis/.append style={
            line width=0.5pt,
            tick style={
                line width=0.5pt,
                color=black
            }
        },
        legend style={
            at={(0.5,1.03)},
            anchor=south,
            legend columns=4,
            font=\small,
            draw=none
        },
        cycle list={
            {blue, mark=none, line width=0.8pt},
            {red, mark=none, line width=0.8pt},
            {green!60!black, mark=none, line width=0.8pt},
            {purple, mark=none, line width=0.8pt}
        }
    }

